Precoding Design for Multi-User MIMO Joint Communications and Sensing

We investigate precoding for multi-user (MU) multiple-input multiple-output (MIMO) joint communications and sensing (JCAS) systems, taking into account the potential interference between sensing and communication channels. We derive indicators for the sensing and communication performance, i.e., the detection probability and the communication signal-to-interference-and-noise ratio (SINR) for general input signals. Our results show that the use of the communication signal for sensing can prevent a loss in communication performance if channel interference occurs, while the kurtosis of the transmit alphabet of the communication signal limits the sensing performance. We present simulation results of example setups.

==> figures/flowgraph_train_new.tex <==
\tikzset{block/.style={rectangle, thick, draw, minimum width=2cm, minimum height=1cm, rounded corners=1.6mm},font=\small,align=center}
\tikzset{crossing/.style={circle, scale=0.4, fill=black}}
\vspace{0.5cm}
%\tikzsetnextfilename{JCaS-flowgraph-train}
\begin{tikzpicture}[node distance=1.5, text=black, >=latex]
	\node[] (start) {$\vect{m} \in \mathcal{M}^{N_{\text{win}}}$};
	\node[block, node distance=0.5cm, right=of start,pattern={north west lines}, pattern color=KITblue!20] (enc){Encoder};
	
	\node[block, below = of enc, fill=KITblue!20] (beam){Beamformer \\ $K$ antennas};
	\node[node distance=0.5cm, left = of beam] (theta){$\theta_{\min},\theta_{\max},$\\$ \varphi_{\min},\varphi_{\max}$};
	
	\node[draw,circle,inner sep=0, radius=0.4cm, thick] (mix) at ($0.5*(beam)+0.5*(enc)+(2,0)$) {\Large{$\times$}} ;
	\node[] (mixtext) at (mix) {};  
	\node[block] (radch) at ($(mix) + (4.2,1.5)$) {Sensing channel:\\ Swerling 1 model};
	\node[block, fill=white,node distance=0.5, right=of radch] (ac) {$\text{Corr}(\mat{z_{\text{s}}},\mat{z_{\text{s}}})$};
	\node[block] (commch) at ($(mix) + (4.2,-1.5)$) {Rayleigh channel};
	\node[crossing] (c1) at ($(mix)+(2.5,0)$){};
	
	\node[draw, minimum size=2cm, rectangle,minimum width = 3cm, minimum height=2.7cm, KITgreen, fill=KITgreen!20,thick, dotted,
	label=south:{Sensing receiver}] (A) at ($(radch)+(6.2,0)$) {};
	
	\node[block, fill=KITblue!20] (detect) at ($(ac) + (3.5,0.7)$) {Target detection};
	
	
	\node[block, fill=KITblue!20] (angle) at ($(ac) + (3.5,-0.7)$) {Angle estimation};
	\node[crossing] (c2) at ($(ac)+(1.5,0)$){};
	%\node[node distance=1.2,below=of c2] (trainangle) {targets};
	\node[node distance=0.5cm, right = of detect] (llr) {${p}_{\text{T}}$};
	\node[node distance=1.2,above=of c2] (traintarg) {targets, $P_{\text{f}}$};
	\node[node distance=0.5cm, right = of angle] (phi) {$\hat{{\theta}}$};
	
	\node[block, fill=KITblue!20] (demod) at ($(commch) + (5,0)$) {Comm. receiver};
	\node (csi) at ($(demod)+(-1.8,-1)$) {CSI $\kappa=\alpha_{\text{c}} \vect{a}_{\text{TX}}^\top(\varphi)\vect{\nu}$};
	%\node[node distance=0.5cm, right = of demod] (bits) {Bitwise LLRs};
	\node[node distance=0.5cm] (bits) at ($(demod.east)-(-1.5,0)$) {Bitwise LLRs\\ $\vect{\ell} \in \mathbb{R}^{\log_2(M) \times N_{\text{win}}}$};
	%\node[node distance=0.5cm] (syms) at ($(demod.east)+(1.18,0.3)$) {$\hat{P}(m|z_{\text{c}})$};
        \node[] (i1) at ($(angle.west)+(-1.4,-0.2)$){$N_{\text{win}}$, $\sigma_{\text{ns}}$};
        \node[] (i2) at ($(detect.west)+(-1.4,0.2)$){$N_{\text{win}}$, $\sigma_{\text{ns}}$};
        \node[] (i3) at ($(demod.west)+(-1.4,-0.2)$){$\sigma_{\text{nc}}$};
 
	\draw[thick, ->] (start) -- (enc);
	\draw[thick, ->] (theta) -- (beam);
	\draw[thick, ->] (beam) -| (mix) node[midway,below] {$\mat{\nu} \in \mathbb{C}^{K\times N_{\text{win}}}$};
	\draw[thick, ->] (enc) -| (mix) node[midway,above] {$\vect{x} \in \mathcal{C}^{N_{\text{win}}}$};
	\draw[thick, ->] (mix) -- (c1) node[midway,above] {$\mat{y}\in \mathbb{C}^{K\times N_{\text{win}}}$} |-  (radch);
	\draw[thick, ->] (mix) -- (c1) |- (commch);
	\draw[thick,->] (radch) -- (ac) node[midway,above]{$\mat{z}_{\text{s}}$};
	\draw[thick] (ac) -- (c2);
	\draw[thick, ->] (c2) |- ($(detect.west)-(0,0.2)$);
	\draw[thick, ->, dashed, KITred] ($(radch.north) + (0.2,0)$) |- (traintarg) -| (detect.north);
	%\draw[thick, ->, dashed, KITred] ($(radch.south) + (0.2,0)$) |- (trainangle) -| (angle);
	%\draw[thick, ->, dashed, KITred] (detect) -- (angle);
	%\draw[thick,->,dashed] ($(enc.north) + (0,0)$) |- ($(radch.north)+(0,1)$) node[near start,black, fill=white] {$x$} -| (detect) -- (angle.north);
	\draw[thick, ->] (c2) |- ($(angle.west)+(0,0.2)$);
	\draw[thick, ->] (detect) -- (llr);
	\draw[thick, ->] (angle) -- (phi);
        \draw[thick, ->] (i2) -- ($(detect.west)-(0,-0.2)$);
        \draw[thick, ->] (i1) -- ($(angle.west)-(0,0.2)$);
        \draw[thick, ->] (i3) -- ($(demod.west)-(0,0.2)$);
	\draw[thick, ->, dashed] (commch) |- (csi) -| (demod);
	\draw[thick, ->] ($(commch.east)+(0,0.2)$) -- ($(demod.west)+(0,0.2)$) node[midway,above]{${\vect{z}}_{\text{c}}$};
	\draw[thick, ->] ($(demod.east)-(0,0)$) -- (bits);
	%\draw[thick, ->] ($(demod.east)+(0,0.3)$) -- (syms);  
	\draw[thick, dashed] (beam.south) |- (commch |- csi);

	
	%\node[node distance=0.3cm, right = of llr,color=KITgreen] (l1) {BCE loss};
	%\node[node distance=0.3cm, right = of phi,color=KITgreen] (l2) {MSE loss};
	%\node[node distance=0.3cm, right = of bits,color=KITgreen] (l3) {BCE loss};
\end{tikzpicture}


==> figures/theober_psk.tex <==
esno ber
0   0.335992121473360
1.000000000000000   0.319009235983479
2.000000000000000   0.301237277326305
3.000000000000000   0.282845555866978
4.000000000000000   0.264023021085621
5.000000000000000   0.244966820713618
6.000000000000000   0.225870782130316
7.000000000000000   0.206916250090423
8.000000000000000   0.188267258933389
9.000000000000000   0.170070708029292
10.000000000000000   0.152460478513750
11.000000000000000   0.135562985343067
12.000000000000000   0.119501132945533
13.000000000000000   0.104394287450790
14.000000000000000   0.090353459083530
15.000000000000000   0.077472782305056
16.000000000000000   0.065819830377020
17.000000000000000   0.055427738537166
18.000000000000000   0.046291427650800
19.000000000000000   0.038368809838205
20.000000000000000   0.031586375921330
21.000000000000000   0.025847572295632
22.000000000000000   0.021042092087938
23.000000000000000   0.017054508931661
24.000000000000000   0.013771275665010
25.000000000000000   0.011085714583374
26.000000000000000   0.008901076331795
27.000000000000000   0.007131997475920
28.000000000000000   0.005704774288161
29.000000000000000   0.004556851218732
30.000000000000000   0.003635851420292
31.000000000000000   0.002898391498123
32.000000000000000   0.002308844402081
33.000000000000000   0.001838151720116
34.000000000000000   0.001462740900953
35.000000000000000   0.001163571949549
36.000000000000000   0.000925318587587
37.000000000000000   0.000735677510663
38.000000000000000   0.000584793527844
39.000000000000000   0.000464786029895
40.000000000000000   0.000369361988479
41.000000000000000   0.000293501598139
42.000000000000000   0.000233204135795
43.000000000000000   0.000185283264670
44.000000000000000   0.000147202643031
45.000000000000000   0.000116944204256

==> figures/theober_qam.tex <==
esno ber
0   0.320515727221482
1.000000000000000   0.301290486059434
2.000000000000000   0.281312888009962
3.000000000000000   0.260783430968155
4.000000000000000   0.239909866686782
5.000000000000000   0.218907430974429
6.000000000000000   0.198001922730853
7.000000000000000   0.177432128292356
8.000000000000000   0.157448008297684
9.000000000000000   0.138302445798532
10.000000000000000   0.120236717003781
11.000000000000000   0.103462308303227
12.000000000000000   0.088143289382884
13.000000000000000   0.074383515276292
14.000000000000000   0.062221489889367
15.000000000000000   0.051633465976151
16.000000000000000   0.042543245948795
17.000000000000000   0.034835911075312
18.000000000000000   0.028372539394740
19.000000000000000   0.023003602763531
20.000000000000000   0.018579697492198
21.000000000000000   0.014959167523061
22.000000000000000   0.012012817573791
23.000000000000000   0.009626251356623
24.000000000000000   0.007700470122543
25.000000000000000   0.006151320885258
26.000000000000000   0.004908270716333
27.000000000000000   0.003912856032064
28.000000000000000   0.003117041738235
29.000000000000000   0.002481635134493
30.000000000000000   0.001974834423966
31.000000000000000   0.001570947847204
32.000000000000000   0.001249291879147
33.000000000000000   0.000993260892870
34.000000000000000   0.000789552392016
35.000000000000000   0.000627528514993
36.000000000000000   0.000498694042966
37.000000000000000   0.000396272287578
38.000000000000000   0.000314862159445
39.000000000000000   0.000250161919012
40.000000000000000   0.000198747298671
41.000000000000000   0.000157893707432
42.000000000000000   0.000125434019891
43.000000000000000   0.000099644991490
44.000000000000000   0.000079156641098
45.000000000000000   0.000062880021986

==> tex_files/attachment.tex <==
\section{Approximation Central limit theorem}

% The expected detection rate can then be calculated as 
% \begin{align}
%     P_{\mathrm{d}} &= \mathbb{E}_{X} \left\{ p\left( \left. \frac{2}{\sigma_{\text{ns}}^2}\sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} |z_{\text{s},il}|^2 > q\chi^2_{2KN_{\text{win}}}(1-P_{\text{f}}) \right|T=1\right)  \right\}\\
%     &= \mathbb{E}_{X} \left\{ p\left( \left. \frac{2K}{\sigma_{\text{ns}}^2}\sum_{l=1}^{N_{\text{win}}} |z_{\text{s},l}|^2 > q\chi^2_{2KN_{\text{win}}}(1-P_{\text{f}}) \right|T=1\right)  \right\}\\ % receive beamforming?
%     % &\approx \frac{1}{M} \left.\sum_{m=1}^{M}p\left(\frac{2KN_{\text{win}}}{\sigma_{\text{ns}}^2} |z_{\text{s},m}|^2 > \chi^2_{2KN_{\text{win}}}(1-P_{\text{f}}) \right|T=1\right)\\  %\frac{1}{M} \sum_{i=1}^{M} \exp\left( \frac{-P_{th}^2}{2|x_i|^2\sigma_{\mathrm{s}}^2+2\sigma_{\mathrm{ns}}^2}\right)
%     % &= \frac{1}{M} \sum_{m=1}^{M} \int_{\ell KN_{\text{win}} |x_l|^2 \sigma_{\text{s}}^2/\sigma_{\text{ns}}^2}^{\infty} \frac{\sigma_{\text{ns}}^2}{2KN_{\text{win}}|x_m|^2\sigma_{\text{s}}^2} \exp\left(-\frac{x\sigma_{\text{ns}}^2}{2KN_{\text{win}}|x_m|^2\sigma_{\text{s}}^2}\right) \delta x \\
%     % &= \frac{1}{M} \sum_{m=1}^{M}  \frac{\sigma_{\text{ns}}^2}{2KN_{\text{win}}|x_m|^2\sigma_{\text{s}}^2} \exp\left(-\frac{x_{th}\sigma_{\text{ns}}^2KN_{\text{win}}|x_m|^2\sigma_{\text{s}}^2}{2KN_{\text{win}}|x_m|^2\sigma_{\text{s}}^2\sigma_{\text{ns}}^2}\right) \\
%     % &= \frac{1}{M} \sum_{m=1}^{M}  \frac{\sigma_{\text{ns}}^2}{2KN_{\text{win}}|x_m|^2\sigma_{\text{s}}^2} \exp\left(-\frac{\chi^2_{2KN_{\text{win}}}(1-P_{\text{f}})}{2}\right)
% \end{align}
% with the quantile of the chi-squared function $q\chi^2(\cdot)$.
% We can get rid of the sum over antennas by applying receive beamforming?
% Are variables along different antennas correlated? YES
% Approximation is exact for $N_{\text{win}}=1$

The weighted sum of multiple chi-squared distributed values doesn't have a closed-form, but with the Imhof method~\cite{Imhof1961}, probabilities can be calculated as exact as necessary. We reformulate the problem as follows:
\begin{align}
    P_d = P\left[ \sum_{l=1}^{N} |x_{l}|^2 \sigma_{\text{s}}^2 |\alpha_l|^2 > \frac{\sigma_{\text{ns}}^2}{2K}q\chi^2_{2KN_{\text{win}}}(1-P_{\text{f}})  \right],
\end{align}
with $|\alpha_l|^2 \in \chi^2_2$.
% comment Imhof method fails for practical values for us often, might not be the right tool for the job

\begin{figure}
    \centering
    %\includegraphics[width=0.5\linewidth]{}
    \begin{tikzpicture}
		\begin{axis}[
			xlabel=$\text{SNR}$ (dB),         ylabel=$P_{\mathrm{d}}$,
			grid=major,
			%legend entries={NN $w_{\text{s}}=0.9$,NN $w_{\text{s}}=0.7$,NN $w_{\text{s}}=0.4$,NN $w_{\text{s}}=0.1$}, 
           legend entries= {QAM, PSK},
			legend cell align={left},
			legend pos=south east,
			xmin=-5,xmax=10,
			%ymin=0.0001,%ymax=4,
			axis line style=thick,
                width=0.95\columnwidth,
                height=0.6\columnwidth,
                legend style={name=leg},
			]
                \addplot[mark=none, color=cb-2, thick] table [ x expr =10*log10(\thisrow{snr}), y = qam]
			{\figures/mimo/my_pd_data.txt};
                \addplot[mark=none, color=cb-3, thick] table [ x expr =10*log10(\thisrow{snr}), y = psk]
			{\figures/mimo/my_pd_data.txt};

\end{axis}
\end{tikzpicture}
    \caption{Example with $N=1$ samples per estimate and $K=16$ antennas for sensing}
    \label{fig:enter-label}
\end{figure}
Similar idea is applied in~\cite{ghatak2025}, maybe also interesting~\cite{Fang2020}.
A different problem is considered in~\cite{Alsusa2013} where the mutliple antenna case matches very well our mathematical scenario.
\begin{itemize}
    \item Create ROC curve (for different x / numer of UEs)
\end{itemize}

Given a MIMO system where the sensing channel is described by
\begin{align}
    \vect{z}_{\text{s}} = T \vect{a}_{\text{RX}}({\theta}) \vect{a}_{\text{TX}}({\theta})^\top \vect{v}^{\top} \vect{x} {\alpha}_{\text{s}} + \vect{n_{\text{s}}},
\end{align}
the optimal detector for an unkown transmit signal is given by
\begin{align}
    \sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} |z_{\text{s},il}|^2 \quad\mathop{\gtreqless}_{\hat{t}=0}^{\hat{t}=1}\quad \underbrace{\frac{\sigma_{\text{ns}}^2}{2}  q\chi^2_{2KN_{\text{win}}}(1-P_{\text{f}})}_{P_{\text{th}}}
\end{align}
We can obtain the scalar values by calculating the diagonal elements of matrix $\vect{z_{\text{s}}}\vect{z_{\text{s}}}^H$ under the assumption that a target is present (T=1):
\begin{align}
    \vect{z_{\text{s}}}\vect{z_{\text{s}}}^H &= |\alpha_{\text{s}}|^2 \vect{a}_{\text{RX}}({\theta}) \underbrace{\vect{a}_{\text{TX}}({\theta})^\top \vect{v}^{\top} \vect{x}}_{\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_t} \vect{x}^H \vect{v}^{*}\vect{a}_{\text{TX}}({\theta})^* \vect{a}_{\text{RX}}({\theta})^H +\notag\\ &\underbrace{\mat{D}}_{\text{mixing terms}} + \vect{n_{\text{s}}}\vect{n_{\text{s}}}^H
\end{align}
with the beamforming gain $\beta_t$ for different transmit signals.The cross-terms in the multiplication are zero-mean and should be negligible as the signal and the noise are uncorrelated. Since $\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_t$ is a scalar, we have associativity in the product. We can reformulate:
\begin{align}
    \vect{z_{\text{s}}}\vect{z_{\text{s}}}^H = |\alpha_{\text{s}}|^2 \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_t\right|^2 \vect{a}_{\text{RX}}({\theta}) \vect{a}_{\text{RX}}({\theta})^H + \mat{D} + \vect{n_{\text{s}}}\vect{n_{\text{s}}}^H
\end{align}
Knowing that $\vect{a}_{\text{RX}}(\varphi)= \left(1,\text{e}^{\j\pi  \sin\varphi},\ldots, \text{e}^{\j\pi (K-1) \sin\varphi}\right)^\top$, the diagonal elements of $\vect{a}_{\text{RX}}(\varphi)\vect{a}_{\text{RX}}(\varphi)^H$ are equal to 1. Therefore, the diagonal elements are given by:
\begin{align}
    |z_{\text{s},il}|^2 = \frac{\sigma_{\text{s}}^2}{2}\underbrace{\frac{2}{\sigma_{\text{s}}^2}|\alpha_{\text{s}}|^2}_{A \in \chi^2_2} \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_t\right|^2  + d_{il} + \frac{\sigma_{\text{ns}}^2}{2}\underbrace{\frac{2}{\sigma_{\text{ns}}^2}|n_{\text{s},i}|^2}_{B \in \chi^2_2}
\end{align}
Note that $\alpha$ is a random variable along the time axis $N_{\text{win}}$, but a constant along the antenna dimension $K$. The same holds for $x_{tl}$ which is randomly chosen from the constellation alphabet of \ac{UE} $t$. Meanwhile, all noise samples $n$ are independant of each other.
\begin{align}
    \sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} |z_{\text{s},il}|^2 &= \sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} \frac{\sigma_{\text{s}}^2}{2}A \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_{tl}\right|^2  + d_{il} + \frac{\sigma_{\text{ns}}^2}{2}B\\
    &= \sum_{l=1}^{N_{\text{win}}} K\frac{\sigma_{\text{s}}^2}{2} \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_{tl}\right|^2A  + d_{il} + \sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} \frac{\sigma_{\text{ns}}^2}{2}B
    \label{eq:starting_point}
\end{align}
We will approximate the mixing terms separately, as they come from a different distribution than the rest of the terms.
They arise from the multiplication of two uncorrelated circular symmetric complex normal distributions. We can express their density as
\begin{align}
    d_il &=  \left(\sum_{t=1}^{N_{\text{UE}}} \sqrt{\beta_t}x_{tl}\right)GE + \left( \left(\sum_{t=1}^{N_{\text{UE}}} \sqrt{\beta_t}x_{tl}\right)GE\right)^*,\\
    GE &= G_1E_1 + \j G_1E_2 + \j G_2E_1 - G_2E_2,
\end{align}
with normal distributions $G_i \in \mathcal{N}(0,\sigma_{\text{s}})$ and $E_i \in \mathcal{N}(0,\sigma_{\text{ns}})$, with
\begin{align}
    f_{G_1\cdot E_1}(z) = \int_{-\infty}^{\infty} \frac{1}{|t|} \left( \frac{1}{\sqrt{2\pi}\sigma_{\text{s}}} \mathrm{e}^{-\frac{t^2}{2 \sigma_{\text{s}}^2}} \right) \left( \frac{1}{\sqrt{2\pi}\sigma_{\text{ns}}} \mathrm{e}^{-\frac{z^2}{2 t^2 \sigma_{\text{ns}}^2}} \right) dt
\end{align}
We can generate the first two moments of this function. Since we add multiple variants of these terms, we can apply the \ac{CLT} and obtain:
\begin{align}
    \sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} d_{il} \in \mathcal{N}\left(0,\sqrt{2N_{\text{win}} K \sigma_{\text{ns}}^2\sigma_{\text{s}}^2\left| \sum_{t=1}^{N_{\text{UE}}} \sqrt{\beta} x_{tl} \right|^2} \right)
\end{align}

% Using the weighted central limit theorem, we can approximate the distribution. Therefore, we first obtain the mean of the distribution:
% \begin{align}
%     \mu = N_{\text{win}} K\sigma_{\text{s}}^2 \mathbb{E}_x \left\{\left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_t\right|^2\right\}   + \ldots + N_{\text{win}} K \sigma_{\text{ns}}^2
% \end{align}
% For simplicity, we assume that only one \ac{UE} illuminates the sensing area while $x$ has normalized power, resulting in 
% \begin{align}
%     \mu = N_{\text{win}} K\sigma_{\text{s}}^2 \beta   + \ldots + N_{\text{win}} K \sigma_{\text{ns}}^2
% \end{align}
According to the weighted central limit theorem~\cite{Weber2006}, we can reformulate the sum of normalized weighted random variables as a normal distribution. Since $\chi^2$-distributions are not centered we start with:
\begin{align}
    A' &= \frac{A-2}{2}, \quad B'=\frac{B-2}{2}\\
    W &= N_{\text{win}}K\sigma_{\text{s}}^2 \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_t\right|^2 +\sum_{l=1}^{N_{\text{win}}} K{\sigma_{\text{s}}^2} \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_t\right|^2 \frac{A-2}{2}  \notag \\ &+ \ldots  + \sigma_{\text{ns}}^2N_{\text{win}}K + \sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} {\sigma_{\text{ns}}^2}\frac{B-2}{2}\\
    &= \underbrace{N_{\text{win}}K\sigma_{\text{s}}^2 \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_t\right|^2 +\sigma_{\text{ns}}^2N_{\text{win}}K}_{\mu'} \notag \\
    &+ \sum_{l=1}^{N_{\text{win}}} K\sigma_{\text{s}}^2 \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_{tl}\right|^2 A'  + \ldots  + \sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} \sigma_{\text{ns}}^2 B'
\end{align}
Now we can apply the weighted central limit theorem to the centralized random variable and shift the normal distribution later by the obtained mean. The weighted central limit theorem states:
\begin{align}
    S_n &= w_1X_1+\ldots + w_nX_n, \quad a_n= w_1^2+ \ldots + w_n^2\\
    S_n/\sqrt{a_n} &\rightarrow \mathcal{N}(0,1)
\end{align}
Under certain conditions that our scenario meets stated in~\cite{Weber2006}
\begin{align}
    \frac{W-\mu'}{\sqrt{a}} \rightarrow \mathcal{N}(0,1), \\
    a= \sum_{l=1}^{N_{\text{win}}} \left(K{\sigma_{\text{s}}^2} \underbrace{\left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_{tl}\right|^2}_{\lambda_l}\right)^2 + \sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} \left({\sigma_{\text{ns}}^2} \right)^2
\end{align}

Using the expectation over $l$ and constraining the launch power using $\mathbb{E}\{ |x_{tl}|^2 \}= N_{\text{win}}$ and $
\sum_{t=1}^{N_{\text{UE}}} |\beta_t| = 1$ with constellations centered around zero $\mathbb{E} \{x_{tl}\}=0$:
\begin{align}
    \lambda &= \mathbb{E}_{x_{tl}\in \mathcal{M}_t} \left\{ \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_{tl}\right|^2\right\}\\
    &=  |\beta_1|\mathbb{E}_l(|x_{1l}|^2) + \ldots + \mathbb{E}_l(\underbrace{2\Re\{\sqrt{\beta_1\beta_2^*}x_{1l}x_{2l}^*\}}_{=0})\\
    &= \sum_{t=1}^{N_{\text{UE}}}|\beta_t| = 1\\
    \tilde{\kappa} &=  \mathbb{E}_{x_{tl}\in \mathcal{M}_t}\left| \sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_{tl}\right|^4 \\
    &= |\beta_1|^2\underbrace{|x_1|^4}_{\kappa_1} + \ldots %+\Re\{\beta_2\beta_2^* \underbrace{x_1^2 (x_2^*)^2}_{E=0, symmetrical constellation}\}
    +4|\beta_1||\beta_2| + \ldots \\
    &= \sum_{t=1}^{N_{\text{UE}}} |\beta_t|^2 \kappa_t + 2|\beta_t|(1-|\beta_t|)\label{eq:kappa}
\end{align}
For this calculation to hold the signals for different \acp{UE} need to be uncorrelated.
% Assuming illumination by one \ac{UE}, this can be rewritten as:
% \begin{align}
%     a = N_{\text{win}}K^2\sigma_{\text{s}}^4 \beta^2 \underbrace{\left|x\right|^4}_{\text{constellation kurtosis } \kappa} + {N_{\text{win}}K\sigma_{\text{ns}}^4} 
% \end{align}
This leads the distribution of $W$ to:
\begin{align}
    W \rightarrow &\mathcal{N}\left(N_{\text{win}}K\sigma_{\text{s}}^2 \lambda +\sigma_{\text{ns}}^2N_{\text{win}}K,\right. \notag\\
    &\left.\sqrt{  {N_{\text{win}}K^2\sigma_{\text{s}}^4} \tilde{\kappa} + {N_{\text{win}}K\sigma_{\text{ns}}^4}}\right)
\end{align}
Combining with the mixed terms, this leads to the approximation:
\begin{align}
    W+D \rightarrow &\mathcal{N}\left(N_{\text{win}}K\sigma_{\text{s}}^2 \lambda +\sigma_{\text{ns}}^2N_{\text{win}}K,\right. \notag\\
    &\left.\sqrt{  {N_{\text{win}}K^2\sigma_{\text{s}}^4} \tilde{\kappa} + {N_{\text{win}}K\sigma_{\text{ns}}^4} +2N_{\text{win}}K\sigma_{\text{ns}}^2\sigma_{\text{s}}^2 \lambda  }\right)
\end{align}

The detection rate is therefore
\begin{align}
    P_{\text{D}} &= P(D+W>P_{\text{th}})\\
    &= 1-\Phi \left(\frac{P_{\text{th}}-N_{\text{win}}K\sigma_{\text{s}}^2 \lambda -\sigma_{\text{ns}}^2N_{\text{win}}K}{\sqrt{{N_{\text{win}}K^2\sigma_{\text{s}}^4} \tilde{\kappa} + {N_{\text{win}}K\sigma_{\text{ns}}^4} + 2N_{\text{win}}K\sigma_{\text{ns}}^2\sigma_{\text{s}}^2 \lambda} }\right)
\end{align}

\subsection{Closed Form Expression for Detection}
Ignoring the ISI terms in \eqref{eq:starting_point}
\begin{align}
    \sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} |z_{\text{s},il}|^2 
    &\approx \underbrace{\sum_{l=1}^{N_{\text{win}}} K\frac{\sigma_{\text{s}}^2}{2} \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_{tl}\right|^2A_l}_{\mathrm{signal-term}}  + \underbrace{\sum_{l=1}^{N_{\text{win}}} \sum_{i=1}^{K} \frac{\sigma_{\text{ns}}^2}{2}B_{il}}_\mathrm{noise-term},
    \label{eq:approximation}
\end{align}
where $A_l$ and $B_{il}$ are independent $\chi^2_2$ variables. The $\chi^2_2$ distribution is the same as the exponential distribution 
\begin{equation}
    f(s;\lambda)=\lambda\mathrm{e}^{-\lambda s}, \quad s\geq 0 
\end{equation}
with rate parameter $\lambda=1/2$ \cite{}. An exponential variable $S\sim\mathrm{Exp}(\lambda)$ with rate parameter $\lambda$ scaled by a scalar $c$ results in an exponential variable with rate parameter $\lambda/c$.

The noise-term in \eqref{eq:approximation} is thus a sum of $N_{\text{win}} \times K$ independent $\mathrm{Exp}(1/\sigma_{\text{ns}}^2)$ variables with joint PDF
\begin{equation}
    f_\mathrm{noise-term}(s)=\frac{\sigma_{\text{ns}}^{-2N_{\text{win}} K} s^{N_{\text{win}} K-1}\mathrm{e}^{-s/\sigma_{\text{ns}}^2}}{(N_{\text{win}} K-1)!}, \quad s\geq 0 
\end{equation}


The signal-term in \eqref{eq:approximation} is then a sum of $N_{\text{win}}$ independent (independence given $x_{tl}$) exponential variables with rate parameters 
\begin{equation}
    \lambda_l=\frac{1}{K\sigma_{\text{s}}^2 \left|\sum_{t=1}^{N_{\text{UE}}}\sqrt{\beta_t} x_{tl}\right|^2}.
\end{equation}
This results in a hypoexponential distribution with PDF
\begin{equation}
    f_\mathrm{signal-term}(s)=\sum_{l=1}^{N_{\text{win}}} \Lambda_l \lambda_l \mathrm{e}^{-\lambda_l s}, \quad s\geq 0,
\end{equation}
where the coefficients $\Lambda_l$ are determined by:
\begin{equation}
    \Lambda_l = \prod_{j=1,\,j\neq l}^{N_{\text{win}}}\frac{\lambda_j}{\lambda_j-\lambda_l}    
\end{equation}


We have two independent random variables:
\begin{itemize}
    \item The signal-term \( S_s \) is hypoexponential:
    \begin{equation}
        f_{S_s}(u) = \sum_{l=1}^{N_{\text{win}}} \Lambda_l \lambda_l e^{-\lambda_l u}, \qquad u \ge 0,
    \end{equation}
    where \( \lambda_l \) are distinct rates and \( \Lambda_l = \prod_{j \neq l} \frac{\lambda_j}{\lambda_j - \lambda_l} \).
    
    \item The noise-term \( S_n \) is gamma:
    \begin{equation}
        f_{S_n}(v) = \frac{\lambda_n^M v^{M-1} e^{-\lambda_n v}}{(M-1)!}, \qquad v \ge 0,
    \end{equation}
    where \( M = N_{\text{win}}K \) and \( \lambda_n = 1/\sigma_s^2 \).
\end{itemize}

The pdf of the sum \( S = S_s + S_n \) is the convolution:
\begin{equation}
    f_S(s) = \int_0^s f_{S_s}(u) f_{S_n}(s - u) \, du.
\end{equation}

---

Substituting \( f_{S_s}(u) \) and \( f_{S_n}(v) \):
\begin{align}
    f_S(s) &= \int_0^s \Bigg( \sum_{l=1}^{N_{\text{win}}} \Lambda_l \lambda_l e^{-\lambda_l u} \Bigg)
    \frac{\lambda_n^M (s - u)^{M-1} e^{-\lambda_n (s - u)}}{(M-1)!} \, du \\
    &= \sum_{l=1}^{N_{\text{win}}} \Lambda_l \lambda_l \frac{\lambda_n^M}{(M-1)!} 
    \int_0^s (s - u)^{M-1} e^{-\lambda_l u} e^{-\lambda_n (s - u)} \, du.
\end{align}

---

Factor out \( e^{-\lambda_n s} \) and define \( \alpha_l = \lambda_l - \lambda_n \):
\begin{align}
    f_S(s) &= \sum_{l=1}^{N_{\text{win}}} \Lambda_l \lambda_l \lambda_n^M e^{-\lambda_n s} \frac{1}{(M-1)!} 
    \int_0^s (s - u)^{M-1} e^{-\alpha_l u} \, du.
\end{align}

Perform the change of variables \( t = s - u \) (thus \( u = s - t \), \( du = -dt \)), limits \( u:0\to s \) map to \( t:s\to0 \):
\begin{align}
    f_S(s) &= \sum_{l=1}^{N_{\text{win}}} \Lambda_l \lambda_l \lambda_n^M e^{-\lambda_n s} \frac{1}{(M-1)!} 
    \int_0^s t^{M-1} e^{-\alpha_l (s - t)} \, dt.
\end{align}

Factor out \( e^{-\alpha_l s} \):
\begin{align}
    f_S(s) &= \sum_{l=1}^{N_{\text{win}}} \Lambda_l \lambda_l \lambda_n^M e^{-\lambda_l s} \frac{1}{(M-1)!} 
    \int_0^s t^{M-1} e^{\alpha_l t} \, dt.
\end{align}

---

The remaining integral is
\begin{equation}
    I_l(s) = \int_0^s t^{M-1} e^{\alpha_l t} \, dt.
\end{equation}

For \( \alpha_l \neq 0 \), this is expressible via the confluent hypergeometric function \( {}_1F_1 \) (Kummer's function):
\begin{equation}
    I_l(s) = \frac{s^M}{M} \, {}_1F_1(M; M+1; \alpha_l s).
\end{equation}

Alternatively, it can also be expressed using the lower incomplete gamma function:
\begin{equation}
    I_l(s) = \frac{\Gamma(M) - \Gamma(M, -\alpha_l s)}{(-\alpha_l)^M}.
\end{equation}

---

Substituting \( I_l(s) \) back into the pdf:
\begin{align}
    f_S(s) &= \sum_{l=1}^{N_{\text{win}}} 
    \Lambda_l \lambda_l \lambda_n^M e^{-\lambda_l s} 
    \frac{s^M}{M(M-1)!} \, {}_1F_1(M; M+1; (\lambda_l - \lambda_n)s), \qquad s \ge 0.
\end{align}

---

\begin{itemize}
    \item When \( \lambda_l = \lambda_n \), the limit \( \alpha_l \to 0 \) must be taken, and the integral reduces to \( I_l(s) = s^M/M \).
    \item For integer \( M \), \( I_l(s) \) can also be written as a finite polynomial times an exponential by expanding \( {}_1F_1 \) in its series form.
\end{itemize}

---
For integer \(M\), expand \( e^{\alpha_l t} \) as a series and integrate term by term:
\[
e^{\alpha_l t} = \sum_{n=0}^\infty \frac{(\alpha_l t)^n}{n!}.
\]
Thus,
\begin{align}
    I_l(s) &= \int_0^s t^{M-1} e^{\alpha_l t} dt 
    = \sum_{n=0}^\infty \frac{\alpha_l^n}{n!} \int_0^s t^{M-1+n} dt \\
    &= \sum_{n=0}^\infty \frac{\alpha_l^n}{n!} \frac{s^{M+n}}{M+n}.
\end{align}

Recognizing this as the series expansion of the confluent hypergeometric function \( {}_1F_1 \):
\begin{equation}
    I_l(s) = \frac{s^M}{M} \, {}_1F_1\!\big(M; M+1; \alpha_l s\big).
\end{equation}

Alternatively, \( I_l(s) \) can be expressed in terms of the lower incomplete gamma function:
\begin{equation}
    I_l(s) = \frac{\Gamma(M) - \Gamma(M, -\alpha_l s)}{(-\alpha_l)^M}.
\end{equation}

---

Substituting \( I_l(s) \) back:
\begin{align}
    f_S(s) &= \sum_{l=1}^{N_{\text{win}}} 
    \Lambda_l \lambda_l \lambda_n^M e^{-\lambda_l s} 
    \frac{s^M}{M(M-1)!} \,
    {}_1F_1\!\big(M; M+1; (\lambda_l - \lambda_n)s\big),
    \qquad s \ge 0.
\end{align}

